The Curious Case of Hallucinatory (Un)answerability: Finding Truths in the Hidden States of Over-Confident Large Language Models

Large language models (LLMs) have been shown to possess impressive capabilities, while also raising crucial concerns about the faithfulness of their responses. A primary issue arising in this context is the management of (un)answerable queries by LLMs, which often results in hallucinatory behavior due to overconfidence. In this paper, we explore the behavior of LLMs when presented with (un)answerable queries. We ask: do models represent the fact that the question is (un)answerable when generating a hallucinatory answer? Our results show strong indications that such models encode the answerability of an input query, with the representation of the first decoded token often being a strong indicator. These findings shed new light on the spatial organization within the latent representations of LLMs, unveiling previously unexplored facets of these models. Moreover, they pave the way for the development of improved decoding techniques with better adherence to factual generation, particularly in scenarios where query (un)answerability is a concern.

==> figures_tex_files/PCA_figures/OPT_2D.tex <==
\begin{figure}[t!]
    \centering
    \setcounter{subfig}{0} % Reset subfig counter

    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/regular_prompt/OPT_squad_2D.png}
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/hint_prompt/OPT_squad_2D.png}
        \stepcounter{subfig} % Increment subfig counter
        \caption{(\alph{subfig}) SQuAD}
        \label{fig:PCA_2D_OPT_SQuAD}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/regular_prompt/OPT_NQ_2D.png}
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/hint_prompt/OPT_NQ_2D.png}
        \stepcounter{subfig} % Increment subfig counter
        \caption{(\alph{subfig}) NQ}
        \label{fig:PCA_2D_OPT_NQ} 
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/regular_prompt/OPT_musique_2D.png}
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/hint_prompt/OPT_musique_2D.png}
        \stepcounter{subfig} % Increment subfig counter
        \caption{(\alph{subfig}) MuSiQue}
        \label{fig:PCA_2D_OPT_MuSiQue} 
    \end{subfigure}

    \caption{2-D PCA projection of the last hidden layer's embedding of the OPT-IML model on each of the three benchmarks. The left images show the embeddings with the regular prompt, and the right ones - with the prompt with a hint.}
    \label{fig:PCA_2D_OPT_full}
\end{figure}

==> figures_tex_files/PCA_figures/T5_2D.tex <==
\begin{figure}[t!]
    \centering
    \setcounter{subfig}{0} % Reset subfig counter

    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/regular_prompt/T5_squad_2D.png}
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/hint_prompt/T5_squad_2D.png}
        \stepcounter{subfig} % Increment subfig counter
        \caption{(\alph{subfig}) SQuAD}
        \label{fig:PCA_2D_T5_SQuAD} 
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/regular_prompt/T5_NQ_2D.png}
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/hint_prompt/T5_NQ_2D.png}
        \stepcounter{subfig} % Increment subfig counter
        \caption{(\alph{subfig}) NQ}
        \label{fig:PCA_2D_T5_NQ}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/regular_prompt/T5_musique_2D.png}
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/hint_prompt/T5_musique_2D.png}
        \stepcounter{subfig} % Increment subfig counter
        \caption{(\alph{subfig}) MuSiQue}
        \label{fig:PCA_2D_T5_MuSiQue} 
    \end{subfigure}

    \caption{2-D PCA projection of the last hidden layer's embedding of the Flan-T5\textsubscript{xxl} model on each of the three benchmarks. The left images show the embeddings with the regular prompt, and the right ones - with the prompt with a hint.}
    \label{fig:PCA_2D_T5_full} 
\end{figure}

==> figures_tex_files/PCA_figures/UL2_2D.tex <==
\begin{figure}[t!]
    \centering
    \setcounter{subfig}{0} % Reset subfig counter

    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/regular_prompt/UL2_squad_2D.png}
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/hint_prompt/UL2_squad_2D.png}
        \stepcounter{subfig} % Increment subfig counter
        \caption{(\alph{subfig}) SQuAD}
        \label{fig:PCA_2D_UL2_SQuAD} 
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/regular_prompt/UL2_NQ_2D.png}
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/hint_prompt/UL2_NQ_2D.png}
        \stepcounter{subfig} % Increment subfig counter
        \caption{(\alph{subfig}) NQ}
        \label{fig:PCA_2D_UL2_NQ} 
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/regular_prompt/UL2_musique_2D.png}
        \includegraphics[width=.45\linewidth]{figures/PCA_2D/hint_prompt/UL2_musique_2D.png}
        \stepcounter{subfig} % Increment subfig counter
        \caption{(\alph{subfig}) MuSiQue}
        \label{fig:PCA_2D_UL2_MuSiQue} %
    \end{subfigure}

    \caption{2-D PCA projection of the last hidden layer's embedding of the Flan-UL2 model on each of the three benchmarks. The left images show the embeddings with the regular prompt, and the right ones - with the prompt with a hint.}
    \label{fig:PCA_2D_UL2_full} 
\end{figure}

==> figures_tex_files/erasure_figures/UL2_squad_2D.tex <==

\begin{figure}[t!]
  \centering

  \begin{subfigure}[b]{0.47\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/PCA_2D/erasure/UL2_squad_no_eraser_2D.png}
    \caption{Before Erasure}

    \label{fig:Erasure_2D_UL2_squad_no_eraser}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.47\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/PCA_2D/erasure/UL2_squad_with_eraser_2D.png}
    \caption{After Erasure}
    \label{fig:Erasure_2D_UL2_squad_with_eraser}
  \end{subfigure}
  
  \caption{2-D PCA projection of the last hidden layer's embedding of the UL2 model on the squad dataset, without performing erasure (left) and after (right).}
  \label{fig:Erasure_UL2_squad_2D}
\end{figure}

==> tables/classifier_results/erasure_classifier.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.4\columnwidth}{!}{%
\begin{tabular}{ll}
\hline
\multicolumn{1}{c}{} & F1 \\ \hline
w\textbackslash{}o eraser & 90.4 \\
with eraser & 61.4 \\ \hline
\end{tabular}%
}
\caption{F1 scores of (un)answerability classification of the linear classifier trained on the embeddings of Flan-UL2 when prompted with SQuAD queries, when tested on the corresponding testset before and after the application of the eraser ("w\textbackslash{}o eraser" and "with eraser", accordingly).}
\label{tab:eraser_F1_classifier}
\end{table}

==> tables/eraser_F1_beam.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[ht!]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{lcc}
\hline
\multicolumn{1}{c}{} & Regular Beam & Relax. Beam \\ \hline
w\textbackslash{}o eraser & 50.1 & 65.4 \\
with eraser & 31.2 & 32.7 \\ \hline
\end{tabular}%
}
\caption{F1 over the (un)answerability classification task with beam relaxation, before and after the application of the concept eraser.}
\label{tab:eraser_F1_beam}
\end{table}

==> tables/old/P_R_F1_few_shot.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|rrrrrrr|rrrrrrr|rrrrrrr|}
\hline
 &  & \multicolumn{7}{c|}{SQuAD} & \multicolumn{7}{c|}{NQ} & \multicolumn{7}{c|}{MuSiQue} \\ \hline
 &  & \multicolumn{3}{l|}{(Un)answerable} & \multicolumn{3}{l|}{Answerable} & \multicolumn{1}{l|}{Accuracy} & \multicolumn{3}{l|}{(Un)answerable} & \multicolumn{3}{l|}{Answerable} & \multicolumn{1}{l|}{Accuracy} & \multicolumn{3}{l|}{(Un)answerable} & \multicolumn{3}{l|}{Answerable} & \multicolumn{1}{l|}{Accuracy} \\ \hline
 &  & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{} \\ \hline
Flan-T5-xxl & Regular & \multicolumn{1}{r|}{99.6} & \multicolumn{1}{r|}{24.4} & \multicolumn{1}{r|}{39.2} & \multicolumn{1}{r|}{56.8} & \multicolumn{1}{r|}{99.9} & \multicolumn{1}{r|}{72.5} & 62.1 & \multicolumn{1}{r|}{97.3} & \multicolumn{1}{r|}{3.2} & \multicolumn{1}{r|}{6.2} & \multicolumn{1}{r|}{31.8} & \multicolumn{1}{r|}{99.8} & \multicolumn{1}{r|}{48.2} & 33.3 & \multicolumn{1}{r|}{95.0} & \multicolumn{1}{r|}{4.3} & \multicolumn{1}{r|}{8.3} & \multicolumn{1}{r|}{60.7} & \multicolumn{1}{r|}{99.8} & \multicolumn{1}{r|}{75.5} & 61.4 \\ \hline
 & +hint (E\&I) & \multicolumn{1}{r|}{93.6} & \multicolumn{1}{r|}{86.8} & \multicolumn{1}{r|}{90.1} & \multicolumn{1}{r|}{87.7} & \multicolumn{1}{r|}{94.0} & \multicolumn{1}{r|}{90.7} & 90.4 & \multicolumn{1}{r|}{87.9} & \multicolumn{1}{r|}{84.7} & \multicolumn{1}{r|}{86.3} & \multicolumn{1}{r|}{68.7} & \multicolumn{1}{r|}{74.2} & \multicolumn{1}{r|}{71.3} & 81.4 & \multicolumn{1}{r|}{75.0} & \multicolumn{1}{r|}{72.6} & \multicolumn{1}{r|}{73.8} & \multicolumn{1}{r|}{81.9} & \multicolumn{1}{r|}{83.6} & \multicolumn{1}{r|}{82.8} & 79.2 \\ \hline
 & +hint (I) & \multicolumn{1}{r|}{94.3} & \multicolumn{1}{r|}{86.0} & \multicolumn{1}{r|}{90.0} & \multicolumn{1}{r|}{87.1} & \multicolumn{1}{r|}{94.8} & \multicolumn{1}{r|}{90.8} & 90.4 & \multicolumn{1}{r|}{89.0} & \multicolumn{1}{r|}{81.9} & \multicolumn{1}{r|}{85.3} & \multicolumn{1}{r|}{66.0} & \multicolumn{1}{r|}{77.6} & \multicolumn{1}{r|}{71.3} & 80.6 & \multicolumn{1}{r|}{78.0} & \multicolumn{1}{r|}{68.1} & \multicolumn{1}{r|}{72.7} & \multicolumn{1}{r|}{80.2} & \multicolumn{1}{r|}{87.1} & \multicolumn{1}{r|}{83.5} & 79.4 \\ \hline
 & +hint (E) & \multicolumn{1}{r|}{96.4} & \multicolumn{1}{r|}{78.0} & \multicolumn{1}{r|}{86.3} & \multicolumn{1}{r|}{81.5} & \multicolumn{1}{r|}{97.1} & \multicolumn{1}{r|}{88.6} & 87.6 & \multicolumn{1}{r|}{91.7} & \multicolumn{1}{r|}{72.7} & \multicolumn{1}{r|}{81.1} & \multicolumn{1}{r|}{58.6} & \multicolumn{1}{r|}{85.4} & \multicolumn{1}{r|}{69.5} & 76.7 & \multicolumn{1}{r|}{89.6} & \multicolumn{1}{r|}{28.3} & \multicolumn{1}{r|}{43.0} & \multicolumn{1}{r|}{66.9} & \multicolumn{1}{r|}{97.8} & \multicolumn{1}{r|}{79.4} & 69.8 \\ \hline
Flan-UL2 & Regular & \multicolumn{1}{r|}{99.7} & \multicolumn{1}{r|}{46.2} & \multicolumn{1}{r|}{63.1} & \multicolumn{1}{r|}{64.9} & \multicolumn{1}{r|}{99.8} & \multicolumn{1}{r|}{78.7} & 73.0 & \multicolumn{1}{r|}{98.0} & \multicolumn{1}{r|}{10.2} & \multicolumn{1}{r|}{18.6} & \multicolumn{1}{r|}{33.4} & \multicolumn{1}{r|}{99.5} & \multicolumn{1}{r|}{50.0} & 38.0 & \multicolumn{1}{r|}{85.9} & \multicolumn{1}{r|}{4.6} & \multicolumn{1}{r|}{8.8} & \multicolumn{1}{r|}{60.7} & \multicolumn{1}{r|}{99.5} & \multicolumn{1}{r|}{75.4} & 61.3 \\ \hline
 & +hint (E\&I) & \multicolumn{1}{r|}{97.2} & \multicolumn{1}{r|}{88.5} & \multicolumn{1}{r|}{92.6} & \multicolumn{1}{r|}{89.4} & \multicolumn{1}{r|}{97.4} & \multicolumn{1}{r|}{93.2} & 93.0 & \multicolumn{1}{r|}{93.2} & \multicolumn{1}{r|}{76.1} & \multicolumn{1}{r|}{83.8} & \multicolumn{1}{r|}{62.4} & \multicolumn{1}{r|}{87.7} & \multicolumn{1}{r|}{72.9} & 79.7 & \multicolumn{1}{r|}{80.7} & \multicolumn{1}{r|}{64.4} & \multicolumn{1}{r|}{71.6} & \multicolumn{1}{r|}{78.8} & \multicolumn{1}{r|}{89.6} & \multicolumn{1}{r|}{83.9} & 79.5 \\ \hline
 & +hint (I) & \multicolumn{1}{r|}{97.5} & \multicolumn{1}{r|}{87.6} & \multicolumn{1}{r|}{92.3} & \multicolumn{1}{r|}{88.7} & \multicolumn{1}{r|}{97.8} & \multicolumn{1}{r|}{93.0} & 92.7 & \multicolumn{1}{r|}{94.0} & \multicolumn{1}{r|}{73.2} & \multicolumn{1}{r|}{82.3} & \multicolumn{1}{r|}{60.2} & \multicolumn{1}{r|}{89.7} & \multicolumn{1}{r|}{72.1} & 78.3 & \multicolumn{1}{r|}{82.0} & \multicolumn{1}{r|}{61.5} & \multicolumn{1}{r|}{70.3} & \multicolumn{1}{r|}{77.8} & \multicolumn{1}{r|}{90.9} & \multicolumn{1}{r|}{83.8} & 79.0 \\ \hline
 & +hint (E) & \multicolumn{1}{r|}{97.6} & \multicolumn{1}{r|}{87.1} & \multicolumn{1}{r|}{92.1} & \multicolumn{1}{r|}{88.3} & \multicolumn{1}{r|}{97.8} & \multicolumn{1}{r|}{92.8} & 92.5 & \multicolumn{1}{r|}{94.6} & \multicolumn{1}{r|}{67.9} & \multicolumn{1}{r|}{79.1} & \multicolumn{1}{r|}{56.3} & \multicolumn{1}{r|}{91.5} & \multicolumn{1}{r|}{69.7} & 75.2 & \multicolumn{1}{r|}{87.0} & \multicolumn{1}{r|}{45.1} & \multicolumn{1}{r|}{59.4} & \multicolumn{1}{r|}{72.0} & \multicolumn{1}{r|}{95.4} & \multicolumn{1}{r|}{82.1} & 75.2 \\ \hline
OPT-IML & Regular & \multicolumn{1}{r|}{98.0} & \multicolumn{1}{r|}{5.7} & \multicolumn{1}{r|}{10.7} & \multicolumn{1}{r|}{51.4} & \multicolumn{1}{r|}{99.9} & \multicolumn{1}{r|}{67.8} & 52.7 & \multicolumn{1}{r|}{98.7} & \multicolumn{1}{r|}{7.2} & \multicolumn{1}{r|}{13.3} & \multicolumn{1}{r|}{32.7} & \multicolumn{1}{r|}{99.8} & \multicolumn{1}{r|}{49.3} & 36.0 & \multicolumn{1}{r|}{93.8} & \multicolumn{1}{r|}{2.3} & \multicolumn{1}{r|}{4.5} & \multicolumn{1}{r|}{60.2} & \multicolumn{1}{r|}{99.9} & \multicolumn{1}{r|}{75.2} & 60.6 \\ \hline
 & +hint (E\&I) & \multicolumn{1}{r|}{83.0} & \multicolumn{1}{r|}{75.7} & \multicolumn{1}{r|}{79.2} & \multicolumn{1}{r|}{77.6} & \multicolumn{1}{r|}{84.5} & \multicolumn{1}{r|}{80.9} & 80.1 & \multicolumn{1}{r|}{83.4} & \multicolumn{1}{r|}{88.9} & \multicolumn{1}{r|}{86.0} & \multicolumn{1}{r|}{71.2} & \multicolumn{1}{r|}{60.8} & \multicolumn{1}{r|}{65.6} & 80.1 & \multicolumn{1}{r|}{80.7} & \multicolumn{1}{r|}{23.6} & \multicolumn{1}{r|}{36.5} & \multicolumn{1}{r|}{65.1} & \multicolumn{1}{r|}{96.2} & \multicolumn{1}{r|}{77.6} & 66.9 \\ \hline
 & +hint (I) & \multicolumn{1}{r|}{88.8} & \multicolumn{1}{r|}{62.8} & \multicolumn{1}{r|}{73.6} & \multicolumn{1}{r|}{71.2} & \multicolumn{1}{r|}{92.1} & \multicolumn{1}{r|}{80.3} & 77.4 & \multicolumn{1}{r|}{89.4} & \multicolumn{1}{r|}{77.6} & \multicolumn{1}{r|}{83.1} & \multicolumn{1}{r|}{61.6} & \multicolumn{1}{r|}{79.6} & \multicolumn{1}{r|}{69.5} & 78.2 & \multicolumn{1}{r|}{87.2} & \multicolumn{1}{r|}{9.8} & \multicolumn{1}{r|}{17.6} & \multicolumn{1}{r|}{61.9} & \multicolumn{1}{r|}{99.0} & \multicolumn{1}{r|}{76.2} & 63.1 \\ \hline
 & +hint (E) & \multicolumn{1}{r|}{96.5} & \multicolumn{1}{r|}{40.2} & \multicolumn{1}{r|}{56.8} & \multicolumn{1}{r|}{62.2} & \multicolumn{1}{r|}{98.5} & \multicolumn{1}{r|}{76.3} & 69.4 & \multicolumn{1}{r|}{95.5} & \multicolumn{1}{r|}{51.6} & \multicolumn{1}{r|}{67.0} & \multicolumn{1}{r|}{46.9} & \multicolumn{1}{r|}{94.6} & \multicolumn{1}{r|}{62.7} & 65.0 & \multicolumn{1}{r|}{81.7} & \multicolumn{1}{r|}{6.8} & \multicolumn{1}{r|}{12.5} & \multicolumn{1}{r|}{61.1} & \multicolumn{1}{r|}{99.0} & \multicolumn{1}{r|}{75.6} & 61.8 \\ \hline
\end{tabular}%
}
\caption{Recall, Precision and F1 scores of answerability and (un)answerability identification, as well as the total accuracy in the few-shot setting. For each ,model, there are four prompt variants: regular, with a hint of the (un)answerability in the exemplars and the instructions ("+hint (E\&I)"), with a hint of the (un)answerability only in the instructions ("+hint (I)"), and with a hint of the (un)answerability only in the exemplars("+hint (E)")}
\label{tab:P_R_F1_few_shot}
\end{table*}

==> tables/old/P_R_F1_zero_shot.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|rrrrrrr|rrrrrrr|rrrrrrr|}
\hline
 &  & \multicolumn{7}{c|}{SQuAD} & \multicolumn{7}{c|}{NQ} & \multicolumn{7}{c|}{MuSiQue} \\ \hline
 &  & \multicolumn{3}{l|}{(Un)answerable} & \multicolumn{3}{l|}{Answerable} & \multicolumn{1}{l|}{Accuracy} & \multicolumn{3}{l|}{(Un)answerable} & \multicolumn{3}{l|}{Answerable} & \multicolumn{1}{l|}{Accuracy} & \multicolumn{3}{l|}{(Un)answerable} & \multicolumn{3}{l|}{Answerable} & \multicolumn{1}{l|}{Accuracy} \\ \hline
 &  & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{} \\ \hline
Flan-T5-xxl & Regular & \multicolumn{1}{r|}{99.7} & \multicolumn{1}{r|}{23.0} & \multicolumn{1}{r|}{37.3} & \multicolumn{1}{r|}{56.4} & \multicolumn{1}{r|}{99.9} & \multicolumn{1}{r|}{72.1} & 61.4 & \multicolumn{1}{r|}{98.3} & \multicolumn{1}{r|}{3.0} & \multicolumn{1}{r|}{5.7} & \multicolumn{1}{r|}{31.8} & \multicolumn{1}{r|}{99.9} & \multicolumn{1}{r|}{48.2} & 33.1 & \multicolumn{1}{r|}{96.6} & \multicolumn{1}{r|}{4.3} & \multicolumn{1}{r|}{8.2} & \multicolumn{1}{r|}{60.7} & \multicolumn{1}{r|}{99.9} & \multicolumn{1}{r|}{75.5} & 61.4 \\ \hline
 & +hint & \multicolumn{1}{r|}{96.6} & \multicolumn{1}{r|}{86.9} & \multicolumn{1}{r|}{91.5} & \multicolumn{1}{r|}{88.0} & \multicolumn{1}{r|}{97.0} & \multicolumn{1}{r|}{92.3} & 91.9 & \multicolumn{1}{r|}{90.7} & \multicolumn{1}{r|}{81.0} & \multicolumn{1}{r|}{85.6} & \multicolumn{1}{r|}{66.0} & \multicolumn{1}{r|}{81.7} & \multicolumn{1}{r|}{73.0} & 81.2 & \multicolumn{1}{r|}{84.4} & \multicolumn{1}{r|}{66.9} & \multicolumn{1}{r|}{74.7} & \multicolumn{1}{r|}{80.4} & \multicolumn{1}{r|}{91.6} & \multicolumn{1}{r|}{85.7} & 81.7 \\ \hline
Flan-UL2 & Regular & \multicolumn{1}{r|}{99.7} & \multicolumn{1}{r|}{30.1} & \multicolumn{1}{r|}{46.3} & \multicolumn{1}{r|}{58.8} & \multicolumn{1}{r|}{99.9} & \multicolumn{1}{r|}{74.0} & 65.0 & \multicolumn{1}{r|}{95.3} & \multicolumn{1}{r|}{7.4} & \multicolumn{1}{r|}{13.8} & \multicolumn{1}{r|}{32.6} & \multicolumn{1}{r|}{99.2} & \multicolumn{1}{r|}{49.1} & 36.0 & \multicolumn{1}{r|}{82.5} & \multicolumn{1}{r|}{3.6} & \multicolumn{1}{r|}{6.8} & \multicolumn{1}{r|}{60.5} & \multicolumn{1}{r|}{99.5} & \multicolumn{1}{r|}{75.2} & 60.8 \\ \hline
 & +hint & \multicolumn{1}{r|}{97.3} & \multicolumn{1}{r|}{87.8} & \multicolumn{1}{r|}{92.3} & \multicolumn{1}{r|}{88.8} & \multicolumn{1}{r|}{97.5} & \multicolumn{1}{r|}{93.0} & 92.6 & \multicolumn{1}{r|}{91.1} & \multicolumn{1}{r|}{77.8} & \multicolumn{1}{r|}{83.9} & \multicolumn{1}{r|}{62.9} & \multicolumn{1}{r|}{83.2} & \multicolumn{1}{r|}{71.6} & 79.5 & \multicolumn{1}{r|}{76.4} & \multicolumn{1}{r|}{60.1} & \multicolumn{1}{r|}{67.3} & \multicolumn{1}{r|}{76.5} & \multicolumn{1}{r|}{87.5} & \multicolumn{1}{r|}{81.6} & 76.5 \\ \hline
OPT-IML & Regular & \multicolumn{1}{r|}{99.4} & \multicolumn{1}{r|}{28.1} & \multicolumn{1}{r|}{43.9} & \multicolumn{1}{r|}{58.1} & \multicolumn{1}{r|}{99.8} & \multicolumn{1}{r|}{73.4} & 63.9 & \multicolumn{1}{r|}{97.6} & \multicolumn{1}{r|}{12.3} & \multicolumn{1}{r|}{21.8} & \multicolumn{1}{r|}{33.9} & \multicolumn{1}{r|}{99.3} & \multicolumn{1}{r|}{50.5} & 39.4 & \multicolumn{1}{r|}{86.2} & \multicolumn{1}{r|}{9.5} & \multicolumn{1}{r|}{17.1} & \multicolumn{1}{r|}{61.8} & \multicolumn{1}{r|}{99.0} & \multicolumn{1}{r|}{76.1} & 62.9 \\ \hline
 & +hint & \multicolumn{1}{r|}{88.9} & \multicolumn{1}{r|}{82.2} & \multicolumn{1}{r|}{85.4} & \multicolumn{1}{r|}{83.4} & \multicolumn{1}{r|}{89.7} & \multicolumn{1}{r|}{86.4} & 85.9 & \multicolumn{1}{r|}{87.8} & \multicolumn{1}{r|}{82.9} & \multicolumn{1}{r|}{85.3} & \multicolumn{1}{r|}{66.3} & \multicolumn{1}{r|}{74.5} & \multicolumn{1}{r|}{70.1} & 80.3 & \multicolumn{1}{r|}{78.0} & \multicolumn{1}{r|}{41.4} & \multicolumn{1}{r|}{54.1} & \multicolumn{1}{r|}{70.0} & \multicolumn{1}{r|}{92.1} & \multicolumn{1}{r|}{79.5} & 71.7 \\ \hline
\end{tabular}%
}
\caption{Recall, Precision and F1 scores of answerability and (un)answerability identification, as well as the total accuracy in the zero-shot setting.}
\label{tab:P_R_F1_zero_shot}
\end{table*}

==> tables/old/classifiers_hint_prompt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cccccccccc|cccccccccc|cccccccccc|}
\hline
{\color[HTML]{333333} } & \multicolumn{10}{c|}{{\color[HTML]{333333} SQuAD}} & \multicolumn{10}{c|}{{\color[HTML]{333333} NQ}} & \multicolumn{10}{c|}{{\color[HTML]{333333} MuSiQue}} \\ \hline
{\color[HTML]{333333} } & \multicolumn{3}{c|}{{\color[HTML]{333333} (un)answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} total}} & {\color[HTML]{333333} Accuracy} & \multicolumn{3}{c|}{{\color[HTML]{333333} (un)answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} total}} & {\color[HTML]{333333} Accuracy} & \multicolumn{3}{c|}{{\color[HTML]{333333} (un)answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} total}} & {\color[HTML]{333333} Accuracy} \\ \hline
{\color[HTML]{333333} } & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & {\color[HTML]{333333} } & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & {\color[HTML]{333333} } & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & {\color[HTML]{333333} } \\ \hline
{\color[HTML]{333333} Flan-T5-xxl} & \multicolumn{1}{c|}{{\color[HTML]{333333} 96}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 84}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 89}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 85}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 96}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 91}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 91}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 90}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 90}} & {\color[HTML]{333333} 90} & \multicolumn{1}{c|}{{\color[HTML]{333333} 92}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 80}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 86}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 66}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 84}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 74}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 79}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 82}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 80}} & {\color[HTML]{333333} 82} & \multicolumn{1}{c|}{{\color[HTML]{333333} 83}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 68}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 75}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 81}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 91}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 85}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 82}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 79}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 80}} & {\color[HTML]{333333} 82} \\ \hline
{\color[HTML]{333333} Flan-UL2} & \multicolumn{1}{c|}{{\color[HTML]{333333} 98}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 73}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 83}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 78}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 98}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 87}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 88}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 85}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 85}} & {\color[HTML]{333333} 85} & \multicolumn{1}{c|}{{\color[HTML]{333333} 96}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 71}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 81}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 59}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 93}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 72}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 77}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 82}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 77}} & {\color[HTML]{333333} 78} & \multicolumn{1}{c|}{{\color[HTML]{333333} 81}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 73}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 77}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 83}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 89}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 86}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 82}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 81}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 81}} & {\color[HTML]{333333} 82} \\ \hline
{\color[HTML]{333333} OPT-IML} & \multicolumn{1}{c|}{{\color[HTML]{333333} 89}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 82}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 86}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 83}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 90}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 87}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 86}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 86}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 86}} & {\color[HTML]{333333} 86} & \multicolumn{1}{c|}{{\color[HTML]{333333} 88}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 84}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 86}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 67}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 74}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 70}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 77}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 79}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 78}} & {\color[HTML]{333333} 81} & \multicolumn{1}{c|}{{\color[HTML]{333333} 91}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 26}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 40}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 57}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 98}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 72}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 74}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 62}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 56}} & {\color[HTML]{333333} 62} \\ \hline
\end{tabular}%
}
\caption{Classifier Recall, Precision and F1 (answerable, (un)answerable and total) and total accuracy scores for each model-data pair, when train on a trainset of 800 answerable and 800 (un)answerable instances when prompt also includes a hint to the possibility of (un)answerability.}
\label{tab:classifier_hint_prompt}
\end{table*}

==> tables/old/classifiers_regular_prompt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cccccccccc|cccccccccc|crrrrrrrrr|}
\hline
{\color[HTML]{333333} } & \multicolumn{10}{c|}{{\color[HTML]{333333} SQuAD}} & \multicolumn{10}{c|}{{\color[HTML]{333333} NQ}} & \multicolumn{10}{c|}{{\color[HTML]{333333} MuSiQue}} \\ \hline
{\color[HTML]{333333} } & \multicolumn{3}{c|}{{\color[HTML]{333333} (un)answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} total}} & \multicolumn{1}{l|}{{\color[HTML]{333333} Accuracy}} & \multicolumn{3}{c|}{{\color[HTML]{333333} (un)answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} total}} & \multicolumn{1}{l|}{{\color[HTML]{333333} Accuracy}} & \multicolumn{3}{c|}{{\color[HTML]{333333} (un)answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} answerable}} & \multicolumn{3}{c|}{{\color[HTML]{333333} total}} & \multicolumn{1}{l|}{{\color[HTML]{333333} Accuracy}} \\ \hline
{\color[HTML]{333333} } & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{l|}{{\color[HTML]{333333} }} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{l|}{{\color[HTML]{333333} }} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{c|}{{\color[HTML]{333333} P}} & \multicolumn{1}{c|}{{\color[HTML]{333333} R}} & \multicolumn{1}{c|}{{\color[HTML]{333333} F1}} & \multicolumn{1}{l|}{{\color[HTML]{333333} }} \\ \hline
{\color[HTML]{333333} Flan-T5-xxl} & \multicolumn{1}{c|}{{\color[HTML]{333333} 95}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 26}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 41}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 57}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 99}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 72}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 76}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 62}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 57}} & {\color[HTML]{333333} 62} & \multicolumn{1}{c|}{{\color[HTML]{333333} 98}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 20}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 33}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 36}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 99}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 53}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 67}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 59}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 43}} & {\color[HTML]{333333} 44} & \multicolumn{1}{r|}{{\color[HTML]{333333} 99}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 12}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 21}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 63}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 100}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 77}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 81}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 56}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 49}} & {\color[HTML]{333333} 64} \\ \hline
{\color[HTML]{333333} Flan-UL2} & \multicolumn{1}{c|}{{\color[HTML]{333333} 99}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 62}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 76}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 72}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 99}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 83}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 85}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 80}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 80}} & {\color[HTML]{333333} 80} & \multicolumn{1}{c|}{{\color[HTML]{333333} 92}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 71}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 80}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 57}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 86}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 69}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 75}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 79}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 74}} & {\color[HTML]{333333} 76} & \multicolumn{1}{r|}{{\color[HTML]{333333} 91}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 54}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 68}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 76}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 96}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 85}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 83}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 75}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 76}} & {\color[HTML]{333333} 79} \\ \hline
{\color[HTML]{333333} OPT-IML} & \multicolumn{1}{c|}{{\color[HTML]{333333} 97}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 48}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 64}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 65}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 99}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 79}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 81}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 73}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 71}} & {\color[HTML]{333333} 73} & \multicolumn{1}{c|}{{\color[HTML]{333333} 95}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 52}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 68}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 47}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 94}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 63}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 71}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 73}} & \multicolumn{1}{c|}{{\color[HTML]{333333} 65}} & {\color[HTML]{333333} 65} & \multicolumn{1}{r|}{{\color[HTML]{333333} 96}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 20}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 33}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 65}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 99}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 78}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 81}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 60}} & \multicolumn{1}{r|}{{\color[HTML]{333333} 56}} & {\color[HTML]{333333} 67} \\ \hline
\end{tabular}%
}
\caption{Classifier Recall, Precision and F1 (answerable, (un)answerable and total) and total accuracy scores for each model-data pair, when train on a trainset of 800 answerable and 800 (un)answerable instances with the regular prompt.}
\label{tab:classifier_regular_prompt}
\end{table*}

==> tables/old/few_shot_answerable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccc}
\hline
 & Method & SQuAD & NQ & \multicolumn{1}{l}{Musique} \\ \hline
Flan-T5-xxl & standard & 92.0 & 78.4 & 73.5 \\
\textbf{} & + hint (examples\&instr.) & 88.4 & 61.0 & 63.0 \\
\textbf{} & + hint (instr.) & 88.9 & 63.5 & 65.8 \\
 & + hint (examples) & 90.9 & 68.5 & 71.8 \\ \hline
Flan-UL2 & standard & 94.9 & 72.3 & 70.5 \\
 & + hint (examples\&instr.) & 93.4 & 72.2 & 69.3 \\
 & + hint (instr.) & 93.7 & 73.7 & 70.1 \\
 & + hint (examples) & 93.6 & 70.7 & 73.5 \\ \hline
OPT-IML & standard & 89.8 & 77.1 & 62.7 \\
\textbf{} & + hint (examples\&instr.) & 78.5 & 51.6 & 62.3 \\
\textbf{} & + hint (instr.) & 84.4 & 64.3 & 62.8 \\
 & + hint (examples) & 88.8 & 73.8 & 63.1 \\ \hline
\end{tabular}%
}
\caption{F1 scores of models' replies when prompted with answerable questions in a Few-Shot setting. Each model is prompted with a standard prompt, a prompt that hints at the possibility of (un)answerability via the instructions and one of the exemplars ("+ hint (examples\&instr.)"), a prompt that hints at the possibility of (un)answerability only through the instructions ("+ hint (instr.)"), and a prompt that hints at the possibility of (un)answerability only through one of the examples ("+ hint (examples.)").}
\label{tab:answerability_few_shot}
\end{table}

==> tables/old/few_shot_un-answerable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccc}
\hline
 & Method & SQuAD & NQ & \multicolumn{1}{l}{Musique} \\ \hline
\multirow{5}{*}{Flan-T5-xxl} & standard & 24.4 & 3.4 & 4.3 \\
 & + hint (examples\&instr.) & 86.8 & 84.7 & 88.6 \\
 & + hint (instr.) & 86.0 & 81.9 & 86.2 \\
 & + hint (examples) & 78.0 & 72.8 & 74.9 \\
 & 2-step & 82.1 & 63.3 & 83.5 \\ \hline
\multirow{5}{*}{Flan-UL2} & standard & 46.2 & 10.3 & 4.7 \\
 & + hint (examples\&instr.) & 88.5 & 76.1 & 80.2 \\
 & + hint (instr.) & 87.6 & 73.2 & 79.4 \\
 & + hint (examples) & 87.1 & 67.9 & 68.0 \\
 & 2-step & 88.0 & 75.6 & 80.5 \\ \hline
\multirow{5}{*}{OPT-IML} & standard & 5.7 & 7.2 & 2.3 \\
 & + hint (examples\&instr.) & 75.7 & 88.9 & 80.1 \\
 & + hint (instr.) & 62.8 & 77.6 & 68.8 \\
 & + hint (examples) & 40.2 & 51.6 & 33.8 \\
 & 2-step & 96.9 & 99.3 & 99.9 \\ \hline
\end{tabular}%
}
\caption{Comparative analysis of (un)answerable question identification percentage in a Few-Shot setting with Varied Prompt strategies.}
\label{tab:unanswerability_few_shot}
\end{table}

==> tables/old/zero_shot_answerable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccc}
\hline
 & Method & SQuAD & NQ & \multicolumn{1}{l}{MuSiQue} \\ \hline
Flan-T5-xxl & standard & 94.3 & 80.0 & 78.4 \\
\textbf{} & +hint & 92.3 & 68.2 & 72.9 \\ \hline
Flan-UL2 & standard & 94.7 & 71.2 & 70.2 \\
 & +hint & 93.2 & 67.0 & 63.6 \\ \hline
OPT-IML & standard & 93.2 & 78.9 & 67.9 \\
\textbf{} & +hint & 84.9 & 63.0 & 63.3 \\ \hline
\end{tabular}%
}
\caption{F1 scores of models' replies when prompted with answerable questions in a zero-shot setting. Each model is prompted with a standard prompt and a prompt that hints to the possibility of (un)answerability ("+hint").}
\label{tab:answerability_zero_shot}
\end{table}

==> tables/old/zero_shot_un-answerable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccc}
\hline
 & Method & SQuAD & NQ & \multicolumn{1}{l}{MuSiQue} \\ \hline
\multirow{3}{*}{Flan-T5-xxl} & standard & 23.0 & 3.1 & 4.3 \\
 & +hint & 86.9 & 81.0 & 67.0 \\
 & 2-step & 85.3 & 66.0 & 84.9 \\ \hline
\multirow{3}{*}{Flan-UL2} & standard & 30.1 & 7.5 & 3.7 \\
 & +hint & 87.8 & 77.8 & 60.1 \\
 & 2-step & 87.4 & 68.1 & 82.4 \\ \hline
\multirow{3}{*}{OPT-IML} & standard & 28.1 & 12.3 & 9.5 \\
 & +hint & 82.2 & 82.9 & 41.4 \\
 & 2-step & 94.2 & 89.2 & 99.0 \\ \hline
\end{tabular}%
}
\caption{Percentage of (un)answerable question identification for the Flan-T5-xxl, Flan-UL2 and OPT-IML models, when the models are being prompted in a zero-shot setting. Each model is prompted with a standard prompt, a prompt that hints to the possibility of (un)answerability ("+hint") and when prompted in a 2-step verification strategy, where the model first prompted to classify the answerability of the question, and only if classified as answerble, asked to answer it.}
\label{tab:unanswerability_zero_shot}
\end{table}
